New Pumping Technique for 2-dimensional VASS

We propose a new pumping technique for 2-dimensional vector addition systems with states (2-VASS) building on natural geometric properties of runs. We illustrate its applicability by reproving an exponential bound on the length of the shortest accepting run, and by proving a new pumping lemma for languages of 2-VASS. The technique is expected to be useful for settling questions concerning languages of 2-VASS, e.g., for establishing decidability status of the regular separability problem.

==> old-defin-of-thick.tex <==
% !TEX root = main.tex
\section{Thin and thick runs}\label{sec:proof}

Our goal is to formulate and prove~\cref{lem:run-2d}, which characterizes the accepting runs in a \nvass{2}.
For this purpose we first define \emph{thin} and \emph{thick} runs.

Let us fix a \nvass{$2$} $V$ with $n$ control states whose  source 
%$s = (p_s, \zero)$ 
and target configurations are $\vec 0$-configurations.
%$t = (p_t, \zero)$.
Let $M = \norm{V}$.

The \emph{belt} of \emph{direction} $v \in \N^2$ and \emph{width} $W$ is the set 
%of all configurations $(q, v)$ with $v$ belonging to the
\[
\belt{v}{W} = \{u \in \N^2 \mid  \dist(u, \ell_v) \leq W \},
\]
where $\dist(u, \ell_v)$ denotes the Euclidean distance between the point $u$ and the half-line $\ell_v$.
We say that a run $\rho$ is \emph{$(A, B)$-thin} if every configuration in $\rho$ belongs to the set 
$Q \times \belt{v}{B}$ for some vector $v$ of norm at most $A$.

%\wojtek{Example of thin run}

In order to formally introduce \emph{thick} runs we need some auxiliary notation.
Consider a sequence of vectors $v_1, \ldots, v_k \in \Z^2$.
We say that a coordinate $j \in \{1, 2\}$ is \emph{dead} at index $i \in \upto{k+1}$ if 
$v_\ell[j] > 0$ for some $\ell < i$; otherwise $j$ is \emph{alive} at $i$. Clearly, both coordinates are alive at 1.
Let $A_i\subseteq \{1,2\}$ be the set of alive coordinates at index $i$; in particular, $A_1 = \{1,2\}$. 
The sequence $v_1, \ldots, v_k$ is \emph{sequentially enabled} in a sequence of
configurations $c_1, \ldots, c_k$ if for every $i \in \upto{k}$ it holds:
\sla{ja w swoim dowodzie zakladam, ze wszystkie wspolrzedne sa dead at $k+1$}
\begin{enumerate}
  \item the $A_{i}$-projection of $v_i$ is nonnegative, i.e., ${(v_i)}_{A_i} \in \N^{A_i}$;
  \item there is a cycle $\pi_i$ with $\eff(\pi_i) = v_i$ which is $A_i$-enabled in $c_i$ (in such case
  we briefly say that the vector $v_i$ itself is $A_i$-enabled in $c_i$).
\end{enumerate}
Intuitively, we relax the requirement that all the cycles $\pi_1, \ldots, \pi_k$ should be
enabled in configurations $c_1, \ldots, c_k$: if the effect of $\pi_i$ is positive on some coordinate
then we do not care about this coordinate for the consecutive cycles $\pi_{i+1}, \ldots, \pi_k$.
In particular, as $A_1 = \{1,2\}$ the vector $v_1$ must be non-negative and enabled in $c_1$; 
the alive set at index 2 is $A_2 = \{ j \mid v_1[j] = 0\}$; 
furthermore ${(v_2)}_{A_2}$ is non-negative and $A_2$-enabled in $c_2$; 
the alive set at index 3 is $A_3 = \{ j \mid v_1[j] = 0 \text{ and } v_2[j] = 0\}$; and so on.
Observe that a coordinate $j$ alive at index $i$ necessarily satisfies $v_1[j] = \ldots = v_i[j] = 0$.

We now put some further condition on sequential enabling, and lift this notion to runs.
The sequence $v_1, \ldots, v_k$ is \emph{$E$-sequentially enabled} in a run $\rho$
if the run decomposes into $\rho = \rho_1 \cdots \rho_k \rho_{k+1}$ such that:
\begin{itemize}
  \item $v_1, \ldots, v_k$ is sequentially enabled in the sequence $\trg(\rho_1), \ldots, \trg(\rho_k)$ 
  of target configurations;
  \item for every $i \in \{1, \ldots, k\}$ and coordinate $j \in A_i$ alive at $i$, 
 the coordinate $j$ is bounded by $E$ in the run $\rho_1\ldots\rho_i$.
\end{itemize}
Intuitively, a coordinate can be greater than $E$ only if it is already dead.

The set $\ccangle{u}{v}$, in case when $v, u \in \N^2$ are non-negative, we call a \emph{positive cone}.
The \emph{sequential cone} of a non-empty sequence of vectors $v_1, \ldots, v_k$ is the set of nonnegative vectors 
$v \in {(\R_{\geq 0})}^2$, which we can obtain as a combination $\sum_{i=1}^k a_i v_i$ with nonnegative coefficients $a_i \in \R_{\geq 0}$ such that every partial sum $\sum_{i=1}^j a_i v_i$ is nonnegative.
In particular $v_1$ may be assumed w.l.o.g.~to be non-negative.
Formally we define the sequential cone by induction on the length of the sequence:
\begin{align*}
\poscone(\emptyseq) & \ = \ \{{\vec 0}\} \\   % l_{v_1} \cap (\R_{\geq 0})^2\\
\poscone (v_1, \ldots, v_i) & \ = \ (\poscone(v_1, \ldots, v_{i-1}) + l_{v_i}) \cap (\R_{\geq 0})^2
\end{align*}
with '+' denoting the Minkowski sum of two sets. 
We stress that the vectors $v_2, \ldots, v_k$ are not necessarily nonnegative.
We easily see:
%
\begin{claim}
The sequential cone of a non-empty sequence of vectors is a positive cone.
\end{claim}
%
%\[
%\poscone(v_1, \ldots, v_k) = \{ \sum_{i=1}^k a_i v_i  \mid a_1, \ldots, a_k \in \R_{\geq 0} \text{ and }
%\forall_{j \leq k} \sum_{i=1}^j a_i v_i \in {(\R_{\geq 0})}^2 \},
%\]
%

An accepting run $\rho$ is \emph{$(C, D, E)$-thick} if $\rho = \rho_1 \rho_2$ such that
\begin{itemize}
  \item there is a sequence of vectors $v_1, \ldots, v_k \in \Z^2$, where $k \leq C$ and $\norm{v_i} \leq D$ 
  for all $i$, which is $E$-sequentially enabled in $\rho_1$;
  \item there is a sequence of vectors $u_1, \ldots, u_l \in \Z^2$, where $l \leq C$ and $\norm{u_i} \leq D$ 
  for all $i$, which is $E$-sequentially enabled in $\rev(\rho_2)$ (in the \twovass $\rev(V)$);
  \item the intersection $\poscone(v_1, \ldots, v_k) \cap \poscone(u_1, \ldots, u_m)$ is a nontrivial positive cone.
  \end{itemize}

\begin{remark}  \label{rem:thick_wlog}
W.l.o.g.~we can assume that at least one coordinate is dead at index 2 in $v_1, \ldots, v_k$ 
(and similarly in $u_1, \ldots, u_k$) -- otherwise, the first vector $v_1 = \vec 0$ can be removed.
Furthermore, w.l.o.g.~we can assume that both coordinates are dead already at index $3$.
Indeed, suppose otherwise that, say, the first coordinate is dead at index while the second coordinate
is still alive at index 3. Thus $v_2$ is necessarily zero on the second coordinate, and therefore $v_2$ 
can be removed, irrespectively of its value on the first coordinate, without compromising the thickness condition.
\end{remark}


\paragraph{\bf Alernative direct definition:}

Three vectors $v_1, v_2, v_3$ we call \emph{sequentially positive} if 
either (1) $v_1$ is positive, or (2) $v_1$ is semi-positive, hence $v_1[j] = 0$ for exactly one $j\in\{1,2\}$, 
and $v_2[j] > 0$. The vectors $v_1, v_2, v_3$ are \emph{sequentially enabled} in a run $\rho$ if this run
partitions into $\rho = \rho_1 \, \rho_2 \, \rho_3 \, \bar \rho$ so that:
\begin{itemize}
\item a cycle with effect $v_1$ is enabled in $c_1 := \trg(\rho_1)$,
\item if $v_1$ is not positive (hence $v_1[j] = 0$) then  a cycle with effect $v_2$ is $\{j\}$-enabled in $c_2$,
otherwise a cycle with effect $v_2$ is $\emptyset$-enabled in $c_2 := \trg(\rho_2)$,
\item a cycle with effect $v_3$ is $\emptyset$-enabled in $c_3 := \trg(\rho_3)$.
\end{itemize}
The vectors $v_1, v_2, v_3$ are \emph{$E$-sequentially enabled} in $\rho$ if 
$c_1[1] \leq E$, $c_1[2] \leq E$, and if $v_1$ is not positive then $c_2[j] \leq E$.
%
Finally, an accepting run $\tau$ we call \emph{(D,E)-thick} if this run partitions into $\tau = \rho \, \rho'$ so that
\begin{enumerate}
\item some vectors $v_1, v_2, v_3$ of norm at most $D$ are $E$-sequentially enabled in $\rho$,
\item some vectors $v'_1, v'_2, v'_3$ of norm at most $D$ are $E$-sequentially enabled in $\rev(\rho')$,
\item $\poscone(v_1, v_2, v_3) \cap \poscone(v'_1, v'_2, v'_3)$ is a nontrivial positive cone.
\end{enumerate}
 
Here is the underlying idea. Denote by $\pi_i$ the cycle enabled in the configuration $c_i$ of $\rho$ 
as required above,
and by ${\pi_1}^j$ the run from $c_1$ induced by the $j$-fold iteration of $\pi_1$.
Point 1
 implies that the cycle $\pi_1$ may be executed arbitrary many times yielding, for every $j\geq 1$, a run
\[
\rho_1 \, {\pi_1}^j \, \rho_2 
\]
from $\src(\tau)$ to a target configuration ${\geq} c_2$; and when $j$ increases towards $+\infty$, 
at least one coordinate of the target configuration diverges towards $+\infty$.
Furthermore, executing in addition $f(j)$-many times the cycle $\pi_2$
(where $f:\N\to\N$ is some linear function) yields, for every $j \geq 1$, a run
\begin{align} \label{eq:runto}
\rho_1 \, {\pi_1}^j \, \rho_2 \, {\pi_2}^{f(j)} \rho_3
\end{align}
to a target configuration ${\geq} c_3$ such that, when $j$ increases towards $+\infty$,
both coordinates of the target configuration diverge from $c_3$ towards $(+\infty, +\infty)$. 
%
Symmetrically, point 2 implies that for every $j\geq 1$ there is a run
\begin{align} \label{eq:runfrom}
\rho'_3 \, {\pi_2}^{f(j)} \, \rho'_2 \, {\pi_1}^{j} \rho'_1
\end{align}
from a source configuration ${\geq} c'_3$ to $\trg(\tau)$ such that when $j$ increases towards $+\infty$,
both coordinates of the source configuration diverge from $c'_3 := \src(\rho'_3)$ towards $(+\infty, +\infty)$. 
%
Finally, point 3 ensures, intuitively, that the directions of divergence of the target configuration of~\eqref{eq:runto}
and the source configuration of~\eqref{eq:runfrom} can be adapted by the cycles $\pi_3$ and $\pi'_3$, respectively,
so that they intersect.


  
%\wojtek{Example of thick run}

\begin{lemma}\label{lem:run-2d}
There is a polynomial $p$ such that for every \twovass $V$  of norm M with $n$ states, 
%and source and target zero configurations, 
every accepting run is either $(A, B)$-thin or $(C, D, E)$-thick for some numbers $A, B, D, E \leq p(n, M^n)$ and $C \leq 4$.
\end{lemma}

\begin{proof}
Sketch goes like that. Assume that $\rho$ is not $(A, B)$-thin. Take some configuration $c$, which is outside of belts and split
$\rho$ in $c$ into $\rho_1$ and $\rho_2$. Apply \cref{lem:positive-approximation} to $\rho_1$, we have that $c \in C_1 = \poscone(v_1, \ldots, v_k)$, where $v_1, \ldots, v_k$ are enabled in $\rho_1$.
Configuration $c$ was taken such that no vector with norm at most $A$ is linearly dependent with $c$. So cone $C_1$
contains also some other vectors around $c$. Similarly apply \cref{lem:positive-approximation} to reverse of $\rho_2$, denoted
$\rev(\rho_2)$. We get that $c \in C_2 = \poscone(u_1, \ldots, u_m)$, where $u_1, \ldots, u_m$ are enabled on $\rho_2$.
Similarly as before we know that $C_2$ has to contain some vectors around $c$. So $C_1 \cap C_2 \neq \emptyset$ and
moreover contains more than a half-line.
\qed
\end{proof}

Thus it remains to show the following lemma.

\begin{lemma}\label{lem:positive-approximation}
Let $\rho$ be a run in $V$ with source $s = (p_s, \zero)$ and target $t = (p_t, v_t)$.
There are polynomials $P$ and $Q$ such that $\rho$ $P(n,M)$-sequentially enables sequence of vectors $v_1, \ldots, v_k \in \Z^2$ with $k \leq 4$ such that $\norm{v_i} \leq P(n,M)$ for all $i \in \{1, \ldots, k\}$ such that
some vector $v \in \N^2$ with $\norm{v-v_t} \leq Q(n,M)^n$ belongs to the positive cone $\poscone(v_1, \ldots, v_k)$.
\end{lemma}

The rest of this section is devoted to proof of \cref{lem:positive-approximation}. We develop slowly, in a sequence of lemmas,
understanding how runs in \nvass{$2$} can look like. 
Let $\Zneg = \Z \setminus \N$ and $\Znonpos = \Z \setminus \N_+$.


\input{proof-lemma}





==> overview.tex <==
% !TEX root = main.tex
\section{Overview}
